FLIQS: One-Shot Mixed-Precision Floating-Point and Integer Quantization Search

Quantization has become a mainstream compression technique for reducing model size, computational requirements, and energy consumption for modern deep neural networks (DNNs). With improved numerical support in recent hardware, including multiple variants of integer and floating point, mixed-precision quantization has become necessary to achieve high-quality results with low model cost. Prior mixed-precision methods have performed either a post-training quantization search, which compromises on accuracy, or a differentiable quantization search, which leads to high memory usage from branching. Therefore, we propose the first one-shot mixed-precision quantization search that eliminates the need for retraining in both integer and low-precision floating point models. We evaluate our search (FLIQS) on multiple convolutional and vision transformer networks to discover Pareto-optimal models. Our approach improves upon uniform precision, manual mixed-precision, and recent integer quantization search methods. With integer models, we increase the accuracy of ResNet-18 on ImageNet by 1.31% and ResNet-50 by 0.90% with equivalent model cost over previous methods. Additionally, for the first time, we explore a novel mixed-precision floating-point search and improve MobileNetV2 by up to 0.98% compared to prior state-of-the-art FP8 models. Finally, we extend FLIQS to simultaneously search a joint quantization and neural architecture space and improve the ImageNet accuracy by 2.69% with similar model cost on a MobileNetV2 search space.

==> sections/sec-checklist.tex <==
\section*{Submission Checklist}

\begin{enumerate}
\item For all authors\dots
  %
  \begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately
    reflect the paper's contributions and scope? \answerYes{the listed contributions are supported throughout the paper}
  \item Did you describe the limitations of your work? \answerYes{In Figure 1 comparing to prior work}
  
  \item Did you discuss any potential negative societal impacts of your work? \answerYes{in the Broader Impact Statement}
  \item Did you read the ethics review guidelines and ensure that your paper
    conforms to them? \url{https://2022.automl.cc/ethics-accessibility/}
    \answerYes{}
  \end{enumerate}
  %
\item If you ran experiments\dots
  %
  \begin{enumerate}
  \item Did you use the same evaluation protocol for all methods being compared (e.g.,
    same benchmarks, data (sub)sets, available resources)?
    \answerYes{}
  \item Did you specify all the necessary details of your evaluation (e.g., data splits,
    pre-processing, search spaces, hyperparameter tuning)?
    \answerYes{In the Appendix}
  \item Did you repeat your experiments (e.g., across multiple random seeds or splits) to account for the impact of randomness in your methods or data?
  \answerYes{Listed the variance for different runs}
  \item Did you report the uncertainty of your results (e.g., the variance across random seeds or splits)?
  \answerYes{}
  \item Did you report the statistical significance of your results?
  \answerYes{the variance captures the significance}
  \item Did you use tabular or surrogate benchmarks for in-depth evaluations?
  Unclear
  \item Did you compare performance over time and describe how you selected the maximum duration?
  Unclear
  \item Did you include the total amount of compute and the type of resources
    used (e.g., type of \textsc{gpu}s, internal cluster, or cloud provider)?
    \answerYes{Mentioned TPU usage in Pareto section}
  \item Did you run ablation studies to assess the impact of different
    components of your approach?
    \answerYes{In the Appendix}
  \end{enumerate}
  %
\item With respect to the code used to obtain your results\dots
  %
  \begin{enumerate}
\item Did you include the code, data, and instructions needed to reproduce the
    main experimental results, including all requirements (e.g.,
    \texttt{requirements.txt} with explicit versions), random seeds, an instructive
    \texttt{README} with installation, and execution commands (either in the
    supplemental material or as a \textsc{url})?
        \answerYes{Included in Supplemental}

  \item Did you include a minimal example to replicate results on a small subset
    of the experiments or on toy data?
   \answerYes{Included in Supplemental}
  \item Did you ensure sufficient code quality and documentation so that someone else
    can execute and understand your code?
   \answerYes{Included in Supplemental}

  \item Did you include the raw results of running your experiments with the given
    code, data, and instructions?
   \answerYes{Included in Supplemental}

  \item Did you include the code, additional data, and instructions needed to generate
    the figures and tables in your paper based on the raw results?
  \answerNo{}

  \end{enumerate}
  %
\item If you used existing assets (e.g., code, data, models)\dots
  %
  \begin{enumerate}
  \item Did you cite the creators of used assets?
\answerYes{Citations throughout paper}
  \item Did you discuss whether and how consent was obtained from people whose
    data you're using/curating if the license requires it?
\answerYes{}
  \item Did you discuss whether the data you are using/curating contains
    personally identifiable information or offensive content?
\answerNo{Not relevant}
  \end{enumerate}
  %
\item If you created/released new assets (e.g., code, data, models)\dots
  %
  \begin{enumerate}
    %
    \item Did you mention the license of the new assets (e.g., as part of your code submission)?
\answerNo{Not relevant}
    \item Did you include the new assets either in the supplemental material or as
    a \textsc{url} (to, e.g., GitHub or Hugging Face)?
\answerNo{Not relevant}
  \end{enumerate}
  %
\item If you used crowdsourcing or conducted research with human subjects\dots
  %
  \begin{enumerate}
  \item Did you include the full text of instructions given to participants and
    screenshots, if applicable?
\answerNo{Not relevant}
  \item Did you describe any potential participant risks, with links to
    Institutional Review Board (\textsc{irb}) approvals, if applicable?
\answerNo{Not relevant}
  \item Did you include the estimated hourly wage paid to participants and the
    total amount spent on participant compensation?
\answerNo{Not relevant}
  \end{enumerate}
\item If you included theoretical results\dots
  %
  \begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
\answerYes{}
  \item Did you include complete proofs of all theoretical results?
\answerYes{}
  \end{enumerate}
  %
\end{enumerate}

==> sections/sec-impact.tex <==
\section{Broader Impact Statement}

After careful reflection, the authors have determined that this work presents no notable
negative impacts to society or the environment.


==> tables/tab-area-fpga-int.tex <==
\begin{table}[tbhp]
    \caption[AreaFpga]
    {\textbf{ResNet-18 Estimated Area} -- Accuracy vs. Area estimates for uniform bitwidth and FLIQS-L variants of ResNet-18. Look-up Tables (LUTs) (measured in thousands) are the fundamental resource on FPGA platforms. Precision represents the precision of the three layers in the ResNet-18 downsampling block: 3$\times$3, 3$\times$3, 1$\times$1.}
    \vspace{5pt}
    \centering
    \small
    \begin{tabular}{@{}cccccc@{}}
    \toprule
    \textbf{Method} & \textbf{Prec.} & \textbf{LUTs (K)} & \textbf{Rel. $\times$} & \textbf{GBOPS} &  \textbf{Top-1}\\
    \toprule
    4B      & 4,4,4 & 42.8 & 1.00$\times$ & 29 & 67.31\\
    5B      & 5,5,5 & 44.8 & 1.05$\times$ & 45 & -\\
    6B      & 6,6,6 & 48.3 & 1.13$\times$ & 65 & -\\
    7B      & 7,7,7 & 54.9 & 1.28$\times$ & 89 & -\\
    8B      & 8,8,8 & 67.6 & 1.58$\times$ & 117 & 70.78\\
    \midrule
    FLIQS-L & 5,5,6 & 45.9& 1.07$\times$ & 46 & 70.12\\
    FLIQS-L & 5,6,6 & 47.1 & 1.10$\times$ & 67 & 70.51\\
    \bottomrule
    \end{tabular}%
    \vspace{0.1in}
    \label{tab:r18-area-fpga}
\end{table}


==> tables/tab-comparison.tex <==
\begin{table}[t]
\caption[Comparison Details]{\textbf{Comparison Details} -- Further method details for related quantization and quantization search works.
}
\vspace{5pt}
\centering
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\small
\begin{tabular}{ccc}
\toprule
\textbf{Method} & \textbf{Mode} & \textbf{Precision}\\
\toprule
HAWQ-V3~\cite{yao2021hawqv3} & PTQ & 4* \\
EDMIPS~\cite{cai2020EDMIPS} & QAT & [1,4] \\
PACT~\cite{choi2018pact} & QAT & 4* \\
AdaQuant~\cite{hubara2020calibtip} & PTQ & 4* \\
LQNets~\cite{zhang2018lqnets} & QAT & 4* \\
INT FLIQS-S & QAT & 4,8,16 \\
INT FLIQS-L & QAT & {[4,8],16} \\
\midrule
HAWQ-V3~\cite{yao2021hawqv3} & PTQ & 4, 8* \\
DQ~\cite{uhlich2020dq} & PTQ & [2,10] \\
PACT~\cite{choi2018pact} & QAT & 5* \\
INT FLIQS-S & QAT & 4,8,16 \\
INT FLIQS-L & QAT & {[4,8],16} \\
\midrule
HFP8~\cite{sun2019hybrid} & PTQ & 8* \\
MPFP~\cite{mellempudi2019mixed} & QAT & 8* \\
FPQuant~\cite{kuzmin2022fp8} & QAT & 8 \\
S2FP8~\cite{cambier2020shifted} & QAT & 8 \\
FP134~\cite{lee2022toward} & QAT & 8 \\
FP FLIQS-S & QAT & 4,8,16 \\
FP FLIQS-L & QAT & {[4,8],16} \\
\bottomrule
\end{tabular}%
\label{tab:comparison}
\end{table}

==> tables/tab-search-ablation.tex <==
\begin{table}[tbhp]
    \caption[Search]{\textbf{Search Characteristics} -- Characteristics of various searches. `Model Cost $\Delta$` represents the average absolute deviation from the target model cost over six targets in [25, 150]. $Cost_L$ represents a quantization search, and $Cost_S$ is a smaller search. Both are in units of GBOPs.}
    \centering
    \small
    \begin{tabular}{c|c|c|c}
    \toprule
    \textbf{Method} & \textbf{$Cost_S\Delta$} & \textbf{$Cost_L \Delta$} & \textbf{Time}\\
    \toprule
    25\% & 8.80 & 14.25 & 40\%\\
    50\% & 5.94 & 6.82 & 80\%\\
    75\% & 4.94 & 5.67 & 127\%\\
    100\% & 4.02 & 4.68 & 146\%\\
    \midrule
    Random & 19.08 & 24.6 & 92\%\\
    \end{tabular}
    \vspace{0.1in}
    \label{tab:search-characteristics}
\end{table}


==> tables/tab-vs-inception.tex <==
\begin{table}[h]
    \caption{\textbf{InceptionV3}}
    \vspace{0.1in}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    \textbf{Format} & \textbf{0.5}$\times$ & \textbf{0.75}$\times$ & \textbf{1.0}$\times$ & \textbf{1.25}$\times$ & \textbf{1.5x}$\times$ \\
    \toprule
    E4M3 & 70.87 & 74.29 & 75.80 & \textbf{76.75 }& \textbf{77.35}\\
    E5M2 & 70.38 & 73.78 & 75.50 & 76.35 & 77.03\\
    INT8 & \textbf{70.98} & \textbf{74.34} & \textbf{75.85} & - & 77.19\\
    \end{tabular}%
    \label{tab:vs-inc}
\end{table}


==> tables/tab-vs-mobile.tex <==
\begin{table}[h]
    \caption{\textbf{MobileNetV2}}
    \vspace{0.1in}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    \textbf{Format} & \textbf{0.25}$\times$ & \textbf{0.5}$\times$ & \textbf{1.0}$\times$ & \textbf{1.4}$\times$ & \textbf{2.0}$\times$ \\
    \toprule
    E4M3 & 55.35 & \textbf{65.62} & \textbf{73.19} &\textbf{ 76.01} & \textbf{77.79}\\
    E5M2 & 53.61 & 63.61 & 72.08 & 75.35 & 77.31\\
    INT8 & \textbf{54.94} &\textbf{ 65.62} & \textbf{73.19} & 75.76 & 77.29\\
    \midrule
    Float & 54.78 & 65.65 & 72.89 & 76.03 & 77.60\\
    \end{tabular}%
    \label{tab:vs-mb}
\end{table}


==> tables/tab-vs-res18.tex <==
\begin{table}[h]
    \caption{\textbf{ResNet18} -- Comparing 8-bit formats: INT8, E4M3, and E5M2. Results are drawn from multiple model widths and the best non-full-precision model is highlighted in \textbf{bold}.}
    \vspace{0.1in}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    \textbf{Format} & \textbf{0.5}$\times$ & \textbf{0.75}$\times$ & \textbf{1.0}$\times$ & \textbf{1.25}$\times$ & \textbf{1.5}$\times$ \\
    \toprule
    E4M3 & 62.05 & \textbf{67.65} & 70.68 & 72.55 & 73.71\\
    E5M2 & 61.31 & 67.01 & 70.16 & 72.27 & 73.46\\
    INT8 & \textbf{62.42} & 67.54 & \textbf{70.78} & \textbf{72.61} & \textbf{73.83}\\
    \midrule
    Float & 62.69 & 68.23 & 71.22 & 73.04 & 74.09\\
    \end{tabular}%
    \label{tab:vs-res18}
\end{table}


==> tables/tab-vs-res50.tex <==
\begin{table}[h]
    \caption{\textbf{ResNet50}}
    \vspace{0.1in}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    \textbf{Format} & \textbf{0.5}$\times$ & \textbf{0.75}$\times$ & \textbf{1.0}$\times$ & \textbf{1.25}$\times$ & \textbf{1.5}$\times$ \\
    \toprule
    E4M3 & 72.95 & \textbf{75.85} & 77.12 & 78.05 & \textbf{78.43}\\
    E5M2 & 72.55 & 75.48 & 76.90 & 77.81 & 78.22\\
    INT8 & \textbf{73.07} & \textbf{75.85} & \textbf{77.28} & \textbf{78.16} & 78.41\\
    \midrule
    Float & 73.85 & 76.29 & 77.45 & 78.17 & 78.67\\
    \end{tabular}%
    \label{tab:vs-res50}
\end{table}

